Online Marketplace: A Benchmark for Data Management in Microservices

Microservice architectures have become a popular approach for designing scalable distributed applications. Despite their extensive use in industrial settings for over a decade, there is limited understanding of the data management challenges that arise in these applications. Consequently, it has been difficult to advance data system technologies that effectively support microservice applications. To fill this gap, we present Online Marketplace, a microservice benchmark that highlights core data management challenges that existing benchmarks fail to address. These challenges include transaction processing, query processing, event processing, constraint enforcement, and data replication. We have defined criteria for various data management issues to enable proper comparison across data systems and platforms. Through case studies with state-of-the-art data platforms, we discuss the issues encountered while implementing and meeting Online Marketplace's criteria. By capturing the overhead of meeting the key data management requirements that are overlooked by existing benchmarks, we gain actionable insights into the experimental platforms. This highlights the significance of Online Marketplace in advancing future data systems to meet the needs of microservice practitioners.

==> sections/97_related.tex <==
\section{Related Work}

% Benchmarking is of utmost importance to the database systems community. 

% This section reviews related work on benchmarks and differentiates them from \OM\ benchmark presented in this work.

% \noindent\textbf{OLTP benchmarks} 
% Online Transaction Processing (OLTP) 

% \noindent\textbf{OLAP benchmarks} 

% microservice benchmarks
% DeathStar benchmark~\cite{deathstar} was created to investigate the effects of microservice architectures on hardware and software in system stacks, particularly network and operating systems.
% TrainTicket~\cite{train_tse} is another benchmark designed to replicate industrial faults in microservices, supporting researchers in fault analysis and debugging. However, while both benchmarks reflect certain aspects of microservice architectures such as functional decomposition and isolation of resources, they fail to address the emerging data management challenges encountered in practice, such as query processing, event processing correctness, data replication, constraints spanning across microservices. Furthermore, they did not clearly specify issues related to transactional guarantees and data invariants, making it difficult to improve data systems for microservice applications.

% google ecommerce benchmark ~\cite{google}
% eshoponcontainers~\cite{eShopOnContainers} and other open source repositories~\cite{instana}

% Similarly, transactional guarantees, data invariants, performance metrics, and message correctness semantics are not a core concern of the study and remain unclear how TrainTicket can effectively support the design of futuristic data systems aimed at microservices.
% Although few invariants are mentioned, 
% " The user is allowed to change the ticket before the departure time or within a certain time period after the train departs"
% performance metrics, transactional guarantees unclear
% message correctness semantics in regard to processing order and delivery semantics



% https://www.tpc.org/tpcw/tpc-w_wh.pdf
TPC-W~\cite{tpcw} is a transactional benchmark that models the core aspects of user experience on an e-commerce website, such as browsing pages, checking out books, and searching for keywords (e.g., by title). %It suggests a traditional tiered architecture with four services: a web server, a web cache, an image server, and a database server. It was discontinued in 2005. 
TPC-C~\cite{tpcc} was designed to represent the transaction processing requirements of a wholesale supplier. YCSB~\cite{ycsb} models transactional workloads in the cloud that are not necessarily executed under ACID semantics. All of them assume a traditional monolithic application architecture. Our benchmark models a modern microservice-oriented application and the complex interplay of their components through events, differing substantially from these benchmarks in terms of architectural style and data management requirements.
% do not capture emerging data management challenges
% In this work, although modeling cart functionality, our work offers a microservice event-driven application and key data management features brought about

Unibench~\cite{unibench} offers OLTP and OLAP workloads for multi-model databases. However, it does not model the decomposition of microservices, which results in the absence of distributed and encapsulated states as found in microservice applications. On the other hand, stream processing benchmarks like Linear Road~\cite{linear_road} focus on modeling continuous and historical queries, but they do not include transactional workloads.

% future work, exploring different deployment schemes in the benchmark
% https://twitter.com/alexxubyte/status/1590384986011549696
% how resilient they are in the presence of failures and continuous deployment?

% BI benchmark in VLDB
% https://www.vldb.org/pvldb/vol16/p877-szarnyas.pdf

% multi-model benchmark vldb
% https://www.vldb.org/pvldb/vol16/p747-moon.pdf



% future work must embrace dynamic workloads
% what we are not doing in this work:
% schema changes, continuous deployment
% dynamic workloads?
% backpressure
% security aspects
% observability
% future work. privacy issues. workload involving customer data removal.

